Slowing Down for Performance and Energy: An OS-Centric Study in Network Driven Workloads

This paper studies three fundamental aspects of an OS that impact the performance and energy efficiency of network processing: 1) batching, 2) processor energy settings, and 3) the logic and instructions of the OS networking paths. A network device's interrupt delay feature is used to induce batching and processor frequency is manipulated to control the speed of instruction execution. A baremetal library OS is used to explore OS path specialization. This study shows how careful use of batching and interrupt delay results in 2X energy and performance improvements across different workloads. Surprisingly, we find polling can be made energy efficient and can result in gains up to 11X over baseline Linux. We developed a methodology and a set of tools to collect system data in order to understand how energy is impacted at a fine-grained granularity. This paper identifies a number of other novel findings that have implications in OS design for networked applications and suggests a path forward to consider energy as a focal point of systems research.

==> conclusion.tex <==
\label{sec:conc}
